PAGnol: An Extra-Large French Generative Model

Access to large pre-trained models of varied architectures, in many different languages, is central to the democratization of NLP. We introduce PAGnol, a collection of French GPT models. Using scaling laws, we efficiently train PAGnol-XL (1.5B parameters) with the same computational budget as CamemBERT, a model 13 times smaller. PAGnol-XL is the largest model trained to date for the French language. We plan to train increasingly large and performing versions of PAGnol, exploring the capabilities of French extreme-scale models. For this first release, we focus on the pre-training and scaling calculations underlining PAGnol. We fit a scaling law for compute for the French language, and compare it with its English counterpart. We find the pre-training dataset significantly conditions the quality of the outputs, with common datasets such as OSCAR leading to low-quality offensive text. We evaluate our models on discriminative and generative tasks in French, comparing to other state-of-the-art French and multilingual models, and reaching the state of the art in the abstract summarization task. Our research was conducted on the public GENCI Jean Zay supercomputer, and our models up to the Large are made publicly available.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = emnlp2021

# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = Ethics.tex draft_final.tex
#1Discussion.tex Intro_Djame.tex









#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).tex
	$(TEX) $(latexfile).tex 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	bibtex $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef
	cat $(latexfile).log | grep --text multipl

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: $(latexfile).pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex  & 


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp:
#	TEMP := $(shell mktemp -u)
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours/$(latexfile)_$(shell gdate +%F_%R).pdf

final: pdf 
	cp $(latexfile).pdf ./PAGnolXL.pdf
	

ebib:
	open $(latexfile).bib


split: bib
	splitappendix $(latexfile).pdf 12
	open -a Skim.app submission.pdf appendix.pdf
	

